Expand More, Shrink Less: Shaping Effective-Rank Dynamics for Dense Scaling in Recommendation

Scaling recommendation models is a central challenge in recommender systems. Recently, RankMixer has emerged as an effective solution, operating on a unified token representation and alternating between token mixing and per-token feedforward networks (P-FFNs) to achieve scalable performance. However, RankMixer suffers from \textit{embedding collapse}, where learned representations have low effective rank, limiting expressivity and underutilizing the expanded representation space. Through empirical analysis and theoretical insights, we identify rigid token mixing and P-FFN modules as the primary causes of this phenomenon, jointly inducing a \textbf{damped oscillatory trajectory} in effective-rank evolution across layers. To address it, we propose RankElastor, a novel architecture that produces spectrum-robust representations with provable collapse mitigation. RankElastor introduces two components: (i) \textbf{parameterized full mixing}, which enables expressive token mixing with improved spectral robustness; and (ii) \textbf{GLU-improved P-FFNs}, which stabilize representation spectra through GLU-style FFN modules. Extensive experiments on large-scale industrial datasets demonstrate that RankElastor consistently improves recommendation performance, mitigates embedding collapse, and exhibits robust scaling behavior. Code is available at this GitHub repository: https://github.com/vasile-paskardlgm/RankElastor

==> sections/method_camera_ready.tex <==
\section{Method: \unimixer}
\label{sec:method}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/unimixer.pdf}
  \caption{Architectural overview of (\textbf{a}) \rankmixer and (\textbf{b}) \unimixer. \underline{\textcolor{mypurple}{Purple}} modules indicate trainable components, while \underline{\textcolor{mygray}{Gray}} modules indicate non-parametric components. The key difference between the models lies in token-mixing and P-FFNs.}
  \label{fig:arch}
\end{figure*}

In this section, we present \unimixer, a novel deep recommender architecture that generalizes the token-mixing and P-FFN modules of \rankmixer through establishing collapse-robust token transformation. 
We focus on two core architectural components in \unimixer: (\textbf{\romannumeral1}) \textit{Parameterized Full Token Mixing} and (\textbf{\romannumeral2}) \textit{GLU-improved P-FFNs}, both supported by theoretical justification. 
An overview of \unimixer is illustrated in Figure~\ref{fig:arch}(\textbf{b}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Parameterized Full Token Mixing}\label{sec:method:full-mixing}
In \rankmixer, token mixing is implemented as a non-parameteric block-transposed operation. 
This operation is equivalent to
\begin{align}
\label{eq:rankmixer-mixing}
\operatorname{vec}(M^\top) = \operatorname{LN}\big((P\otimes I)\operatorname{vec}(X^\top) + \operatorname{vec}(X^\top)\big)\ ,
\end{align}
where \(P \in \mathbb{R}^{T^2 \times T^2}\) is a permutation operator structured as a \textit{commutation matrix}~\cite{commutation-matrix}, \(I\in\mathbb{R}^{\frac{D}{T}\times\frac{D}{T}}\) denotes the identity matrix, \(\operatorname{vec}\) denotes the \textit{vec operator}~\cite{vec-operator}, \(\operatorname{LN}\) denotes layer normalization, and \(\otimes\) is the \textit{Kronecker product}~\cite{matrix-analysis}.

This representation reveals an important structural property: token mixing is governed by the permutation operator \(P\) and the grid scale \(d = \frac{D}{T}\). 
Modifying either the permutation operator or the grid scale leads to different token-mixing behaviors. 
Motivated by this observation, we generalize Eq.~\ref{eq:rankmixer-mixing} by introducing a learnable mixing operator and reducing the grid scale to the finest resolution. 
This leads to the proposed \textbf{parameterized full mixing}:
\begin{align}
\label{eq:full-mixing}
\operatorname{vec}(M^\top) = \operatorname{LN}\big((W + I)\operatorname{vec}(X^\top)\big)\ ,
\end{align}
where \(W\in\mathbb{R}^{TD\times TD}\) is a learnable mixing matrix and \(I\) preserves residual information flow.

This formulation corresponds to the fine-grained case \(d=1\) with fully parameterized mixing weights, enabling interactions across all token–feature coordinates. 
Such generalization strengthens the token-mixing module by allowing the model to refine representations that may otherwise lead to spectral collapse under restricted block-wise transformations. 
We formalize this expressivity advantage in the following theorem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Expressivity of parameterized full mixing]
\label{thm:parameterized-block-mixing}
Let $X\in\mathbb R^{T\times D}$ be an input representation matrix and $x=\operatorname{vec}(X)\in\mathbb{R}^{N}$ with $N=TD$. For a divisor $d^{\ast}$ of $N$, partition $x$ into $K=N/d^{\ast}$ blocks $\mathcal{B}=\{\mathbf{b}_1,\dots,\mathbf{b}_K\}$, where $\mathbf{b}_k\in\mathbb{R}^{d^{\ast}}$. A parameterized block-mixing scheme with learnable weights $\mathbf{W}\in\mathbb{R}^{K\times K}$ produces \(\mathbf{y}=(\mathbf{W}\otimes\mathbf{I}_{d^{\ast}})\,\mathbf{x} \) and the residual output \(\mathbf{C} =\Phi_{d^{\ast}}(\mathbf{X};\mathbf{W}) \triangleq \mathbf{X} +\operatorname{reshape}\!\left( (\mathbf{W}\otimes\mathbf{I}_{d^{\ast}})\operatorname{vec}(\mathbf{X}) \right).\) Then for any $d^{\ast}>1$, the set of linear transformations realizable by $\Phi_{d^{\ast}}$ is strictly contained in that of the parameterized full mixing case ($d^{\ast}=1$). In particular, the Kronecker constraint $(\mathbf{W}\otimes\mathbf{I}_{d^{\ast}})$ prevents expressing fine-grained, high-rank coordinate interactions that are attainable when $d^{\ast}=1$.
\end{theorem}

The theorem's justification is presented in Appendix. 
The theorem shows that when the grid scale satisfies \(d^{\ast}>1\), there always exist nontrivial inputs whose token-mixing outputs remain spectrally constrained. 
In contrast, the fine-grained case \(d^{\ast}=1\), corresponding to our parameterized full mixing, removes the Kronecker constraint and enables richer coordinate interactions, improving robustness against representational collapse.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{GLU-improved P-FFNs}\label{sec:method:geglu-ffn}
Although parameterized full mixing improves the expressivity of token representations at the matrix level—in terms of effective rank—its collapse mitigation effect is primarily statistical rather than deterministic. 
In practical recommendation scenarios, highly skewed or degenerate inputs may still lead to degraded representations. 
To further improve robustness, we refine the second core module of \rankmixer, namely the P-FFN.

We replace the GELU-based FFN with a GLU-style gated feed-forward module (\textbf{bias omitted for clarity}):
\begin{align}
\label{eq:geglu-ffn}
Z_t = \big(\operatorname{GELU}(M_t W_1)\odot(M_t W_2)\big)W_3 + M_t W_r\ ,
\end{align}
where \(W_1, W_2\in\mathbb{R}^{D\times rD}\) are lifting projections, \(W_3\in\mathbb{R}^{rD\times D}\) is the compression projection, \(r\) is the expansion ratio, \(W_r\) is a learnable residual mapping, and $\odot$ denotes the \textit{Hadamard product}~\cite{linear-algebra}. 
This design follows the gated activation principle of GLU~\cite{GLU-activation}, which has been shown to improve expressivity and representation quality in modern deep architectures~\cite{GLU-llm-1,GLU-llm-2,GLU-llm-3}.

We next show that the GLU-improved P-FFN provides stronger effective rank recovery capability than the GELU-based FFN used in \rankmixer.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Effective rank recovery via GLU-improved P-FFNs]
\label{thm:geglu_recovery}
Let $X\in\mathbb R^{T\times D}$ satisfy $\operatorname{erank}(X)=k$ with $k/D\le \gamma$ for a fixed constant $\gamma\in(0,1)$.  
Consider the GLU-improved P-FFN with residual
\[
\mathcal G(X)=\big(\phi(XA)\odot(XC)\big)B + XD,
\]
where $A,C\in\mathbb R^{D\times m}$ and $B\in\mathbb R^{m\times D}$ have i.i.d.\ sub-Gaussian entries with variance $1/D$, and $\odot$ denotes the Hadamard product. 
If the hidden width satisfies $m \ge C k\log D$, then with probability at least $1-\exp(-c k)$:
\begin{itemize}[leftmargin=15pt,parsep=2pt,itemsep=2pt,topsep=2pt]
    \item (\textbf{Algebraic lifting})  
    The multiplicative term induces degree-2 interactions, and
    \(
    \operatorname{rank}\!\big(\phi(XA)\odot(XC)\big)\;\ge\;\min\!\left(D,\frac{k(k+1)}{2}\right).
    \)
    \item (\textbf{Effective rank increase})  
    The output satisfies
    \(
    \operatorname{erank}(\mathcal G(X)) \ge \operatorname{erank}(X) + \delta,
    \)
    for some $\delta>0$ depending only on $\gamma$ and initialization constants.
\end{itemize}
\end{theorem}

The theorem's justification is presented in Appendix. 
This result shows that GLU-improved P-FFNs can statistically maintain spectrum robustness through multiplicative feature interaction, whereas conventional activation-based FFNs may still exhibit nontrivial failure cases that lead to collapse in effective rank. 
Consequently, the proposed P-FFN improves robustness against representational collapse while maintaining the standard feed-forward computation structure used in \rankmixer.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Complexity Analysis}\label{sec:method:complexity}
We compare \rankmixer and \unimixer via the computational and parameter complexity of token mixing and P-FFN modules.

\subsubsection*{\bf On token mixing.} The token mixing module in \rankmixer is implemented as a block-transpose permutation, which incurs $\mathcal{O}(TD)$ computation and introduces no additional parameters. 
In contrast, \unimixer employs \textbf{Parameterized Full Mixing}, which applies a dense linear transformation over the flattened representation. 
This results in $\mathcal{O}(T^2D^2)$ computation and $\mathcal{O}(T^2D^2)$ parameters.

\subsubsection*{\bf On P-FFN} The P-FFN module in \rankmixer has computational complexity $\mathcal{O}(TrD^2)$ and parameter complexity $\mathcal{O}(rD^2)$. 
The \unimixer P-FFN adopts a \textbf{GLU-improved P-FFN}, which increases the feed-forward cost to $\mathcal{O}\big(T(3rD^2 + D^2)\big)$ with parameter complexity $(3r+1)D^2$. 
This introduces a constant-factor increase compared with the P-FFN in \rankmixer.

Overall, the primary complexity difference between \rankmixer and \unimixer arises from the token-mixing module, where \unimixer introduces additional parameters and computation through Parameterized Full Mixing. 
The GLU-improved P-FFN contributes a smaller, constant-factor increase in complexity.

% \subsection{Implementation notes}
% We implement FullMix as batched GEMMs over heads and use pre-norm for stability.
% We found that learning rate warmup and slightly stronger weight decay on $\mathbf{A}_{\ell}^{(h)}$ improves training stability at scale.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/preliminaries_camera_ready.tex <==
\section{Research Background}
\label{sec:background}

\subsection{Notations and Preliminaries}\label{sec:background:prelim}

Recommendation models aim to predict user actions based on features drawn from multiple fields~\cite{multi-field-categorical-data}. 
In line with the application scenario considered in this paper, namely \textit{CTR/ranking prediction}~\cite{ctr-prediction}, we consider \(n\) fields, where the \(i\)-th field is denoted as \(\mathcal{X}_i\), and define the joint feature space as \(\mathcal{X}=\mathcal{X}_1\times\mathcal{X}_2\times\dots\times\mathcal{X}_n\). 
Let \(\mathcal{Y}\) denote the prediction space; the goal of a recommendation model is to learn a mapping from \(\mathcal{X}\) to \(\mathcal{Y}\).

We focus on recommenders following the ``embedding-interaction'' architecture. 
Such models first transform an input sample \(X \in \mathcal{X}\) into a \textit{\textbf{feature embedding}} \(E \in \mathbb{R}^{n \times k}\), where \(k\) is the embedding dimension and the \(i\)-th row \(E_i\) denotes the embedding vector for field \(i\). 
The embedding matrix is then processed by a \textit{\textbf{feature interaction}} module~\cite{feature-interaction-1,feature-interaction-2}, which models correlations across fields and produces informative representations for prediction. 
This architecture is widely adopted in real-world recommender systems due to its strong empirical performance~\cite{dcnv2+crossnet,xdeepfm+cin,autoint,fm}.

\subsubsection*{\bf Embedding Collapse~\cite{embedding-collapse-1-multiembedding}.} In general machine learning settings, dimensional collapse refers to models degenerating into trivial representations that map inputs to nearly constant outputs~\citep{dimension-collapse}, which can be characterized through spectral analysis of learned representations~\citep{dimension-collapse-svd}. 
In recommender systems, a related phenomenon known as \textit{\textbf{embedding collapse}} has recently been identified: the embedding matrix becomes approximately low-rank with multiple near-zero singular values~\citep{embedding-collapse-1-multiembedding,embedding-collapse-2,embedding-collapse-3,embedding-collapse-4-ulrec}. 

This phenomenon is commonly measured using \textit{effective rank}~\cite{effective-rank}, which characterizes the spectral distribution of a matrix beyond algebraic rank. 
Among several formulations, we adopt a widely used norm-based definition~\cite{norm-erank-1,norm-erank-3,norm-erank-4}, also known as the stable rank~\cite{norm-erank-2}:
\begin{align}\label{eq:norm-erank}
\operatorname{erank}(X) = \frac{\sum_{i}\sigma^2_i}{\max_i\sigma^2_i} 
= \frac{\|X\|_F^2}{\|X\|_2^2}\ ,
\end{align}
where \(\sigma_i\) denotes the singular values of \(X\).

\subsubsection*{\bf \rankmixer~\cite{rankmixer}.} As a recent deep recommender architecture, \rankmixer has attracted substantial attention due to its streamlined design, strong empirical performance, and favorable scaling behavior. 
Its architecture consists of three modules: (\textbf{\romannumeral1}) \textit{tokenization}; (\textbf{\romannumeral2}) \textit{token mixing}; and (\textbf{\romannumeral3}) \textit{per-token FFNs} (P-FFNs). We briefly summarize them below:

\begin{itemize}[leftmargin=15pt,parsep=2pt,itemsep=2pt,topsep=2pt]
    \item {\it \underline{Tokenization}.} The tokenization module takes the embedding matrix \(E\) and groups embedding vectors into \(T\) clusters, followed by a unified projection (e.g., linear mapping or MLP) into a shared \(D\)-dimensional space, producing a token matrix \(X^{(0)}\in\mathbb{R}^{T\times D}\). 
    Each row \(X^{(0)}_t\in\mathbb{R}^D\) is called a token embedding. 
    This module is primarily used for aligning embeddings from heterogeneous sources. 
    In this paper, we focus on the subsequent core modules.
    
    \item \textbf{\textit{\underline{Token mixing}.}} The token mixing module partitions the column dimension \(D\) into \(H\) equal segments of size \(d = D/H\), forming a \(T \times T\) grid of blocks, each in \(\mathbb{R}^{1 \times d}\). 
    At the \(l\)-th \rankmixer block, a block-transpose operation is first applied to the input \(X^{(l)}\), exchanging block pairs \(X^{(l)}_{i,j}\) and \(X^{(l)}_{j,i}\). 
    The transformed representation is then combined with the original token matrix through a residual connection, followed by output layer normalization, producing enhanced token representations with cross-token information mixing.
    
    \item \textbf{\textit{\underline{P-FFNs}.}} \rankmixer then sends the mixed tokens into the token-specific FFN modeuls, which is called P-FFN. 
    This module serves as the function for performing feature interaction as those in typical ``embedding-interaction'' type recommenders. 
    In \rankmixer, the P-FFN is configured as a two layer with GELU~\cite{GELU-activation} as activation function.
\end{itemize}

Stacking token mixing and P-FFN modules yields a deep and scalable recommender architecture. 
An overview of the \rankmixer architecture is shown in Figure~\ref{fig:arch}(\textbf{a}).


\begin{figure*}[t]
  \centering
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_criteo_base_Raw_to_Mixing_1.pdf}
        % \caption{Raw Embedding $\to$ Mixing 1}
        \label{fig:erank-criteo-base-1-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_criteo_base_Mixing_1_to_FFN_1.pdf}
        % \caption{Mixing 1 $\to$ FFN 1}
        \label{fig:erank-criteo-base-2-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_criteo_base_FFN_1_to_Mixing_2.pdf}
        % \caption{FFN 1 $\to$ Mixing 2}
        \label{fig:erank-criteo-base-3-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_criteo_base_Mixing_2_to_FFN_2.pdf}
        % \caption{Mixing 2 $\to$ FFN 2}
        \label{fig:erank-criteo-base-4-rankmixer}
    \end{subfigure}
    \\
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_avazu_base_Raw_to_Mixing_1.pdf}
        \caption{Raw Embedding $\to$ Mixing 1}
        \label{fig:erank-avazu-base-1-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_avazu_base_Mixing_1_to_FFN_1.pdf}
        \caption{Mixing 1 $\to$ FFN 1}
        \label{fig:erank-avazu-base-2-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_avazu_base_FFN_1_to_Mixing_2.pdf}
        \caption{FFN 1 $\to$ Mixing 2}
        \label{fig:erank-avazu-base-3-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/UniMixer_avazu_base_Mixing_2_to_FFN_2.pdf}
        \caption{Mixing 2 $\to$ FFN 2}
        \label{fig:erank-avazu-base-4-rankmixer}
    \end{subfigure}
  % \vskip -0.1in
  \caption{Distributional shift of effective rank across representation stages in \rankmixer. Distributions of per-sample effective rank from raw embeddings to successive module outputs on Criteo (top) and Avazu (bottom).}
  \label{fig:erank-rankmixer}
\end{figure*}

\begin{figure}[t]
  \centering
    \begin{subfigure}{0.495\linewidth}
        \centering
        \includegraphics[width=1.02\linewidth]{figs/erank_rankmixer_vs_baselines_criteo.pdf}
        \caption{Comparison on Criteo.}
        \label{fig:avg-erank-criteo-rankmixer}
    \end{subfigure}
    %
    \begin{subfigure}{0.495\linewidth}
        \centering
        \includegraphics[width=1.02\linewidth]{figs/erank_rankmixer_vs_baselines_avazu.pdf}
        \caption{Comparison on Avazu.}
        \label{fig:avg-erank-avazu-rankmixer}
    \end{subfigure}
    %
  % \vskip -0.05in
  \caption{Comparison of average effective rank across representation stages for \rankmixer (damped oscillatory trajectory) and baselines (monotonic decay).}
  \label{fig:avg-erank-rankmixer}
  % \vskip -0.1in
\end{figure}


\subsection{On Embedding Collapse in \rankmixer}\label{sec:background:collapse-rankmixer}

Although \rankmixer demonstrates strong scalability and effectiveness, its behavior under embedding collapse has not been systematically studied. 
Existing collapse analyses primarily focus on conventional recommenders~\cite{embedding-collapse-1-multiembedding,feagen}, such as DCNv2~\cite{dcnv2+crossnet} and xDeepFM~\cite{xdeepfm+cin}. 
In this section, we analyze the effective-rank dynamics of \rankmixer representations across its core modules (token mixing and P-FFNs), combining empirical observations with theoretical justification.

\subsubsection*{\bf Empirical Demonstrations.} We conduct CTR prediction experiments on two industrial-scale benchmarks, Criteo~\cite{criteo} and Avazu~\cite{avazu}, using the FuxiCTR framework~\cite{benchmark-fuxictr}. 
We compare \rankmixer (with two token-mixing blocks and two P-FFN blocks) against DCNv2 and xDeepFM configured with comparable depth, resulting in four-layer recommenders for fair comparison. 
We then visualize the average effective rank of module outputs across test samples. 
All remaining experimental settings follow those described in Section~\ref{sec:exps}.

While full recommendation performance results are reported in Section~\ref{sec:exps}, we focus here on effective-rank dynamics. 
As shown in Figure~\ref{fig:avg-erank-rankmixer}, conventional models exhibit a \textbf{monotonic decay} in effective rank with depth; in contrast, \rankmixer shows an alternating pattern: token mixing increases effective rank, whereas P-FFNs shrink it, producing a \textbf{damped oscillatory trajectory}. 
Although such sawtooth pattern allows \rankmixer to maintain slightly higher effective rank than conventional models, the improvement remains limited and does not eliminate collapse.

On Criteo, the effective rank at the final layer only marginally exceeds that of the raw embeddings, indicating that the rank-enhancement effect of token mixing is modest in practice. 
This limitation becomes more pronounced on Avazu (Figure~\ref{fig:avg-erank-avazu-rankmixer}), where contractions introduced by P-FFNs dominate across layers, causing collapse to re-emerge despite the presence of token mixing.

Since higher effective rank typically indicates better utilization of representation capacity and correlates with improved recommendation performance~\cite{embedding-collapse-1-multiembedding,feagen}, these results reveal both the advantage and limitation of \rankmixer from the perspective of embedding collapse: although the architecture improves representation rank compared with conventional recommenders, it does not fundamentally prevent collapse.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{\bf Theoretical Justifications.} We further complement the empirical analysis with theoretical justification. 
Both the effective-rank improvement and the remaining collapse limitation of \rankmixer can be traced to its two modules: token mixing and P-FFNs. 
The following theorems provide theoretical justification for these effects.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Effective rank under block-transpose mixing]
\label{thm:erank-bound-blocktranspose}
Let $X\in\mathbb R^{T\times D}$ be a representation matrix with \(D = Td\) and \(d \ge 1\). Partition $X$ into a \( T \times T\) grid of blocks $X_{ij} \in \mathbb{R}^{1\times d}$. Define the block-transpose operator $\mathcal{T}$ by \((\mathcal{T}(X))_{ij}=X_{ji}\), and let $Y = \mathcal{T}(X)$. Denote the algebraic rank and effective rank of $X$ by $\operatorname{rank}(X)=r$ and $\operatorname{erank}(X)=k$. Assume $X$ satisfies Frobenius-orthogonality and spectral incoherence with its block transpose:
\[
\langle X, Y \rangle_F \approx 0 \quad \mathrm{and} \quad \|X+Y\|_{2}^2\approx \max(\|X\|_{2}^2,\|Y\|_{2}^2)\ .
\]
Let $M = X+Y$ and define $\mu = \operatorname{erank}(Y)$. Then
\[
\frac{2k\mu}{(\sqrt{k}+\sqrt{\mu})^2} \le \operatorname{erank}(M) \le 2 (k + \mu)\ ,
\]
where $\mu \le \operatorname{rank}(Y) \le \min\{T, rd\}$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Effective rank failure of standard FFNs]
\label{thm:ffn_failure}
Let $X\in\mathbb R^{T\times D}$ be a representation matrix with effective rank
\(
\operatorname{erank}(X)=k \quad\text{and}\quad \frac{k}{D}\le \gamma,
\)
for some fixed constant $\gamma\in(0,1)$ independent of $D$. 
Consider the per-row feedforward network 
\(
\mathcal F(X)=\phi(XA)B,
\)
where $A\in\mathbb R^{D\times m}$ and $B\in\mathbb R^{m\times D}$ have i.i.d.\ sub-Gaussian entries with variance $1/D$, and $\phi$ is positively homogeneous. 
Then:
\begin{itemize}[leftmargin=15pt,parsep=2pt,itemsep=2pt,topsep=2pt]
    \item (\textbf{Deterministic collapse})  
    If $X$ has an algebraic rank $1$, then
    \(
    \operatorname{rank}(\mathcal F(X))\le 2
    \), and 
    \(
    \operatorname{erank}(\mathcal F(X))\le 2
    \)
    , with equality $=1$ when all rows of $X$ have the same sign.
    \item (\textbf{Probabilistic contraction})  
    If the pre-activations satisfy a nontrivial response-gap condition (See Appendix), then with probability at least $1-\exp(-c k)$,
    \(
    \operatorname{erank}(\mathcal F(X)) \le \alpha\,\operatorname{erank}(X),
    \)
    for some constant $\alpha\in(0,1)$ depending only on $\gamma$ and activation $\phi$.
\end{itemize}
\end{theorem}


Theorem~\ref{thm:erank-bound-blocktranspose} explains why token mixing can increase effective rank. 
The block-transpose mixing produces a representation whose effective rank admits the lower bound
\(
\frac{2k\mu}{(\sqrt{k}+\sqrt{\mu})^2}.
\)
showing that mixing introduces a rank-expansion effect. 
However, the theorem also reveals an intrinsic limitation: the achievable improvement is bounded by
\(
\operatorname{erank}(X+Y)\le 2(k+\mu).
\)
Since recommender embeddings are often already spectrally collapsed at initialization stages~\cite{embedding-collapse-1-multiembedding,embedding-collapse-2,embedding-collapse-5}, this bounded expansion typically results in only modest rank improvement in practice. 
This explains the small rank increase observed after token mixing in Figures~\ref{fig:erank-avazu-base-1-rankmixer} and~\ref{fig:erank-avazu-base-3-rankmixer}.

Theorem~\ref{thm:ffn_failure} characterizes the complementary effect of P-FFNs. 
When the input representation is already low-rank, the FFN module can further contract effective rank, either deterministically in the rank-1 case or probabilistically generic rank-\(k\). 
This explains the repeated effective-rank decreases observed in Figures~\ref{fig:erank-avazu-base-2-rankmixer} and~\ref{fig:erank-avazu-base-4-rankmixer}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{\bf Summary.} Taken together, the empirical and theoretical analyses reveal a consistent picture of spectra dynamics in \rankmixer. 
Although \rankmixer maintains higher effective rank than conventional recommenders, the improvement is inherently limited and does not reliably prevent collapse from re-emerging across layers. 
This limitation arises from the architecture itself: token mixing provides bounded rank expansion, while P-FFNs exhibit rank-contractive behavior, jointly producing the characteristic damped oscillatory trajectory across depth.

Importantly, this diagnosis suggests a principled direction for architectural refinement — \textbf{Expand More and Shrink Less}, enabling token mixing to produce stronger spectrum expansion while making P-FFNs less spectrum-reductive. 
Motivated by this insight, we propose \unimixer in the next section.
